Impact of Massive Binary Star and Cosmic Evolution on Gravitational Wave Observations II: Double Compact Object Rates and Properties

Making the most of the rapidly increasing population of gravitational-wave detections of black hole (BH) and neutron star (NS) mergers requires comparing observations with population synthesis predictions. In this work we investigate the combined impact from the key uncertainties in population synthesis modelling of the isolated binary evolution channel: the physical processes in massive binary-star evolution and the star formation history as a function of metallicity, $Z$, and redshift $z, \mathcal{S}(Z,z)$. Considering these uncertainties we create 560 different publicly available model realizations and calculate the rate and distribution characteristics of detectable BHBH, BHNS, and NSNS mergers. We find that our stellar evolution and $\mathcal{S}(Z,z)$ variations can impact the predicted intrinsic and detectable merger rates by factors $10^2$-$10^4$. We find that BHBH rates are dominantly impacted by $\mathcal{S}(Z,z)$ variations, NSNS rates by stellar evolution variations and BHNS rates by both. We then consider the combined impact from all uncertainties considered in this work on the detectable mass distribution shapes (chirp mass, individual masses and mass ratio). We find that the BHNS mass distributions are predominantly impacted by massive binary-star evolution changes. For BHBH and NSNS we find that both uncertainties are important. We also find that the shape of the delay time and birth metallicity distributions are typically dominated by the choice of $\mathcal{S}(Z,z)$ for BHBH, BHNS and NSNS. We identify several examples of robust features in the mass distributions predicted by all 560 models, such that we expect more than 95% of BHBH detections to contain a BH $\gtrsim 8\,\rm{M}_{\odot}$ and have mass ratios $\lesssim 4$. Our work demonstrates that it is essential to consider a wide range of allowed models to study double compact object merger rates and properties.

==> tables/Fiducial_settings_BPS.tex <==



\begin{table*}
%
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline  \hline
Description and name                                 														& Value/range                       & Note / setting   \\ \hline  \hline
\multicolumn{3}{c}{Initial conditions}                                                                      \\ \hline
Initial mass $\monei$                               															& $[5, 150]$\Msun    & \citet{2001MNRAS.322..231K} IMF  $\propto  {\monei}^{-\alpha}$  with $\alpha_{\rm{IMF}} = 2.3$ for stars above $5$\Msun	  \\
%
Initial mass ratio $\qi = \mtwoi / \monei $           												& $[0, 1]$                          &       We assume a flat mass ratio distribution  $p(\qi) \propto  1$ with \mtwoi $\geq 0.1\Msun$   \\
%
Initial separation $\ai$                                            											& $[0.01, 1000]$\AU & Distributed flat-in-log $p(\ai) \propto 1 / {\ai}$ \\ %We reject  binaries with \ai s.t. there is mass transfer at birth.            \\
%
%
Initial metallicity $\Zi$                                           											& $[0.0001, 0.03]$                 & Distributed using a uniform grid in $\log(\Zi)$ with 53 metallicities        \\
%
Initial orbital eccentricity $\ei$                                 							 				& 0                                & All binaries are assumed to be circular at birth  \\
%
% initial rotation of stars                            															& 0                                 &                  \\  \hline
\hline
%initial mass function (IMF) slope 	$\alpha_{\rm{IMF}}$									&  $ 2.3$		& 	 for stars above $5$\Msun from \citet{2001MNRAS.322..231K} IMF\\  \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% WIND THINGS %%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{3}{c}{Fiducial parameter settings:}                                                            \\ \hline
%
Stellar winds  for hydrogen rich stars                                   																&      \citet{2010ApJ...714.1217B}    &   Based on {\citet{2000A&A...362..295V,2001A&A...369..574V}}, including  LBV wind mass loss with $f_{\rm{LBV}} = 1.5$   \\
%
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}}  Stellar winds for hydrogen-poor helium stars &  \citet{2010ApJ...715L.138B} & Based on   {\citet{1998A&A...335.1003H}} and  {\citealt{2005A&A...442..587V}}  with $f_{\rm{WR}} = 1$  \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% MASS TRANSFER THINGS %%%%%%%%%%%%%%%%%%%%%%%
%
Max transfer stability criteria & $\zeta$-prescription & Based on \citet[][]{2018MNRAS.481.4009V} and references therein     \\ 
%
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} Mass transfer accretion rate & thermal timescale & Limited by thermal timescale for stars  \citet[][]{2018MNRAS.481.4009V,2020MNRAS.498.4705V} \\ 
 & Eddington-limited  & Accretion rate is Eddington-limited for compact objects  \\
%
Non-conservative mass loss & isotropic re-emission &  {\citet[][]{1975MmSAI..46..217M,1991PhR...203....1B,1997A&A...327..620S}} \\ 
& &  {\citet{2006csxs.book..623T}} \\
%
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} Case BB mass transfer stability                                														& always stable         &       Based on  \citet{2015MNRAS.451.2123T,2017ApJ...846..170T,2018MNRAS.481.4009V}         \\ 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% CE THINGS %%%%%%%%%%%%%%%%%%%%%%%
%
CE prescription & $\alpha-\lambda$ & based on  \citet{1984ApJ...277..355W,1990ApJ...358..189D}  \\
%
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} CE efficiency $\alpha$-parameter                     												& 1.0                               &              \\
%
CE $\lambda$-parameter                               													& $\lambda_{\rm{Nanjing}}$                             &        Based on \citet{2010ApJ...716..114X,2010ApJ...722.1985X} and  \citet{2012ApJ...759...52D}       \\
%
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} Hertzsprung gap (HG) donor in \ac{CE}                       														& pessimistic                       &  Defined in \citet{2012ApJ...759...52D}:  HG donors don't survive a \ac{CE}  phase        \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%.    SN THINGS   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ac{SN} natal kick magnitude \vk                          									& $[0, \infty)$\kms & Drawn from Maxwellian distribution with standard deviation $\sigma_{\rm{rms}}^{\rm{1D}}$ for \ac{NS}, down-scaled by the fallback fraction for \ac{BH}          \\
%
 \ac{SN} natal kick polar angle $\thetak$          											& $[0, \pi]$                        & $p(\thetak) = \sin(\thetak)/2$ \\
%
 \ac{SN} natal kick azimuthal angle $\phi_k$                           					  	& $[0, 2\pi]$                        & Uniform $p(\phi) = 1/ (2 \pi)$   \\
%
 \ac{SN} mean anomaly of the orbit                    											&     $[0, 2\pi]$                             & Uniformly distributed  \\
 %
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} Core-collapse  \ac{SN} remnant mass prescription          									     &  delayed                     &  From \citep{2012ApJ...749...91F}, which  has no lower \ac{BH} mass gap  \\%
%
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} USSN  remnant mass prescription          									     &  delayed                     &  From \citep{2012ApJ...749...91F}   \\%
%
ECSN  remnant mass presciption                        												&                                 $m_{\rm{f}} = 1.26\Msun$ &      Based on Equation~8 in \citet{1996ApJ...457..834T}          \\
%
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} Core-collapse  \ac{SN}  velocity dispersion $\sigma_{\rm{rms}}^{\rm{1D}}$ 			& 265\kms           & 1D rms value based on              \citet{2005MNRAS.360..974H}                          \\
%
 USSN  and ECSN  velocity dispersion $\sigma_{\rm{rms}}^{\rm{1D}}$ 							 	& 30\kms             &            1D rms value based on e.g.    \citet{2002ApJ...571L..37P,2004ApJ...612.1044P}    \\
%
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} PISN / PPISN remnant mass prescription               											& \citet{2019ApJ...882...36M}                    &       As implemented in \citet{2019ApJ...882..121S}      \\
{\hspace{-.35cm}\Large{\textcolor{cyan}{$\star$}}}{\hspace{+.02cm}} Maximum NS mass                                      & $\rm{max} \, m_{\rm{NS}} = 2.5$\Msun &             \\
Tides and rotation & & We do not include tides and/or stellar rotation\\
%
%
\hline
\multicolumn{3}{c}{Simulation settings}                                                                     \\ \hline
Total number of binaries sampled per metallicity  & $\approx 10^6$                    &      We simulate about a million binaries per \Zi grid point            \\
Sampling method                                      & \sc{STROOPWAFEL} &                Adaptive importance sampling from  \citet{2019MNRAS.490.5228B}  \\
%
Binary fraction                                      & $f_{\rm{bin}} = 1$ &       Corrected factor to be consistent with e.g. {\citet[][]{2017IAUS..329..110S}}        \\
Solar metallicity \Zsun                             & \Zsun = 0.0142 & based on {\citet{2009ARA&A..47..481A}} \\
Binary population synthesis code                                      & COMPAS &       \citet{stevenson2017formation, 2018MNRAS.477.4685B, 2018MNRAS.481.4009V, 2019MNRAS.490.3740N} \\
& & \citet{2019MNRAS.490.5228B}        \\
%2011IAUS..272..474S, 2015A&A...580A..93D, 2017A&A...598A..84A,
\hline \hline
\end{tabular}%
% \end{adjustbox}
}
\caption{Initial values and default settings of the population synthesis  simulation with {\sc{COMPAS}} for our fiducial model A. More details can be found in \citet{2021arXiv210302608B} and in  the  {\sc{COMPAS}}  methods paper (in prep.).  Cyan star symbols in front of a row indicate prescriptions that we vary. These variations are listed in  Table~\ref{tab:variations-BPS}.  An overleaf latex template for this table that is available for public use can be found at \url{https://github.com/FloorBroekgaarden/templateForTableBPSsettings}.  }
\label{tab:population-synthesis-settings}
\centering
\end{table*}
%


==> tables/bps_models_detail_table.tex <==
%


%
\begin{table*}
%
\resizebox{\textwidth}{!}{%
\centering
\begin{tabular}{|l|lll|rrr|}
\hline \hline
$\mu$ & Label 	& Changed physics & Variation  			&  $\#\rm{BHBH}$    & $\#\rm{BHNS}$ &$\#\rm{NSNS}$	\\ \hline \hline
%
A      & fiducial		& --        		& --     				 & $8\,371\,398$	& $1\,525\,553$   & $233\,137$  	\\
%
%
\hline
%%%%%%%%%%%%%% MASS TRANSFER PHYSICS %%%%%%%%%%%%%% 
%
B     & $\beta =0.25$  		& mass transfer                  				& fixed mass transfer efficiency of $\beta=0.25$  		 &  $8\,616\,008$ & $738\,537$ &  $41\,984$ \\ 
%
C       & $\beta =0.5$  		& mass transfer                  				& fixed mass transfer efficiency of $\beta=0.5$  	 & $6\,568\,454$	& $148\,043$  &  $45\,070$ \\ 
%
D        & $\beta =0.75$ 		& mass transfer                  				& fixed mass transfer efficiency of $\beta=0.75$  	 & $6\,033\,721$
	& $118\,921$ &  $292\,349$   \\ 
%
E       & unstable case BB		& mass transfer 	& case BB mass transfer is always unstable 		 & $9\,274\,636$ 	&   $458\,667$&   $371$  \\
%
F       & E + J	& 	& variation E and J	 & $9\,782\,847$	& $828\,558$  &  $7\,491$   \\
%
\hline
%%%%%%%%%%%%%%  CE PHYSICS %%%%%%%%%%%%%% 
%
G       &$\alpha_{\rm{CE}} = 0.1$		& {CE}                    				&  CE efficiency parameter $\alpha_{\rm{CE}} = 0.5$  & $6\,338\,030$	& $22\,395$	& 	$345\,779$  \\
%
H       &$\alpha_{\rm{CE}} = 0.5$		& {CE}                    				&  CE efficiency parameter $\alpha_{\rm{CE}} = 0.5$  & $7\,958\,497$	& $915\,179$ 	& $64\,260$ 	  \\
%
I        & $\alpha_{\rm{CE}} = 2$			& {CE}                    				& CE efficiency parameter $\alpha_{\rm{CE}} = 2$   & $6\,212\,236$	& 	$833\,433$ & $1\,052\,472$ 	\\
%
J       & $\alpha_{\rm{CE}} = 10$			& {CE}                    				& CE efficiency parameter $\alpha_{\rm{CE}} = 2$   & $3\,514\,443$	& $441\,924$ & $579\,059$	\\
%
K      	& optimistic CE	&  {CE}       		& HG donor stars initiating a CE survive CE     			 & 	$8\,782\,290$	& $1\,535\,042$ &   $234\,963$ 	\\
%
\hline
%%%%%%%%%%%%%%  SN PHYSICS %%%%%%%%%%%%%% 
%
%
L       & rapid SN		& SN                   				& Fryer rapid {SN} remnant mass prescription   	 & $7\,463\,923$	&  $2\,766\,298$ &  $ 146\,467$   \\
%
M      & $\rm{max} \, m_{\rm{NS}} = 2\Msun$		& SN                 				& maximum NS mass is fixed to $2\Msun$   	 & $8\,879\,317$	&  $959\,796$   & $213\,669$    \\
%
N        & $\rm{max} \, m_{\rm{NS}} = 3\Msun$		& SN                 				& maximum NS mass is fixed to $3\Msun$    & 	$7\,906\,131$	& $1\,990\,330$ & $238\,111$  \\
%
O       & no PISN		& SN                   				& we no  PISN and pulsational-PISN  	& $8\,547\,080$	& $1\,524\,497$  & $233\,190$   \\
%
P      	 & SN $\sigma_{\rm{rms}}^{\rm{1D}}=100$\kms 	& SN                 				& $\sigma_{\rm{rms}}^{\rm{1D}}=100$\kms  	for core-collapse {SNe}	& $8\,106\,172$ & $3\,049\,458$ & $415\,335$  \\  
%
Q        & SN $\sigma_{\rm{rms}}^{\rm{1D}}=30$\kms 		& SN                  				& $\sigma_{\rm{rms}}^{\rm{1D}}=30$\kms  	for core-collapse {SNe} & $7\,609\,741$	& $4\,198\,238$  & $626\,019$  \\ 
%
R       & SN $v_{\rm{k,BH}} = 0$		& SN                   				& we assume \acp{BH} receive no natal kick   &	$8\,777\,168$	& $5\,068\,628$  & $155\,208$ \\
\hline
%
%%%%%%%%%%%%%%  CE PHYSICS %%%%%%%%%%%%%% 
%
S       &$f_{\rm{WR}}=0.1$		& {stellar wind}                    				&   wolf-rayet wind factor $f_{\rm{WR}} = 0.1$  & $8\,921\,965$	& $1\,379\,487$ 	& $191\,544$ 	  \\
%
T        & $f_{\rm{WR}}=5$			& {stellar wind}                    				& wolf-rayet wind factor $f_{\rm{WR}} = 5$	    & $6\,748\,472$	& 	$938\,755$ & $276\,279$ 	\\
%
%
\hline \hline
\end{tabular}%
}
\caption{List of the \NmodelsBPS binary population synthesis models studied in this work. $\mu$ and `Label' denote the alphabetical letter and abbreviated name used to label each model, `Changed physics' and `Variation' denote which category of physics and what we changed, respectively. The columns $\#$BHBH, $\#$BHNS and $\#$NSNS quote the total number of data points in the combined simulation over 53 metallicity bins that consist of a \ac{BHNS}, \ac{BHBH} and \ac{NSNS}  systems that merge in a Hubble time, respectively.   The fiducial model settings are summarized in Table~\ref{tab:population-synthesis-settings}.}
\label{tab:variations-BPS-more-detailed}
\centering
\end{table*}
%

